Ultraverse: A System-Centric Framework for Efficient What-If Analysis for Database-Intensive Web Applications

Existing what-if analysis systems are predominantly tailored to operate on either only the application layer or only the database layer of software. This isolated approach limits their effectiveness in scenarios where intensive interaction between applications and database systems occurs. To address this gap, we introduce Ultraverse, a what-if analysis framework that seamlessly integrates both application and database layers. Ultraverse employs dynamic symbolic execution to effectively translate application code into compact SQL procedure representations, thereby synchronizing application semantics at both SQL and application levels during what-if replays. A novel aspect of Ultraverse is its use of advanced query dependency analysis, which serves two key purposes: (1) it eliminates the need to replay irrelevant transactions that do not influence the outcome, and (2) it facilitates parallel replay of mutually independent transactions, significantly enhancing the analysis efficiency. Ultraverse is applicable to existing unmodified database systems and legacy application codes. Our extensive evaluations of the framework have demonstrated remarkable improvements in what-if analysis speed, achieving performance gains ranging from 7.7x to 291x across diverse benchmarks.

==> acminfo.tex <==
\setcopyright{acmlicensed}
\acmJournal{PACMMOD}
\acmYear{2025} \acmVolume{3} \acmNumber{1 (SIGMOD)} \acmArticle{84} \acmMonth{2}\acmDOI{10.1145/3709734}
\received{July 2024}
\received[revised]{September 2024}
\received[accepted]{November 2024}

==> copyright.tex <==
% SIGMOD
% \setcopyright{rightsretained}
% \acmDOI{10.475/123_4}
% \acmISBN{123-4567-24-567/08/06}
% \acmConference[SIGMOD'21]{SIGMOD Conference}{June 2021}{Xi'an, China}
% \acmYear{2021}
% \copyrightyear{2021}
% \acmArticle{4}
% \acmPrice{15.00}


==> evaluation-old.tex <==
\section{Evaluation}
\label{sec:evaluation}




\para{Implementation:} \textcolor{orange}{\ultraverse's query dependency analysis (\autoref{sec:design}) is applicable to unmodified commodity DBMSes if they use SQL to manage databases and can log all committed queries (e.g., MySQL, Postgres, MariaDB). And \ultraverse's SQL transpilation (\autoref{sec:transpiler}) is compatible with general-purpose application programming languages that can be executed by dynamic symbolic execution (e.g., JavaScript, Python, C). Among these vast options, we chose MySQL and JavaScript as the \ultraverse prototype's host DBMS and host application language, due to their widespread popularity.}
We implemented the retroactive DBMS plugin (column-wise \& row-wise dependency analysis, replay scheduler, and Hash-jumper) in C++. The query analyzer reads MySQL's binary log~\cite{mysql-binary-log} to retrieve committed queries and computes each query's $R/W$ sets and table hashes. The replay scheduler uses a lockless queue~\cite{lockless-queue} and atomic compare-and-swap instructions ~\cite{compare-and-swap} to reduce contention among threads simultaneously dequeuing the queries to replay. For database rollback, there are 3 options: \textit{(i)} sequentially apply an inverse operation to every committed query; \textit{(ii)} use a temporal database to stage all historical table states; \textit{(iii)} assume periodic snapshots of backup DBs (e.g., every 3 days, 1 week). Our evaluation chose option 3 as it is the easiest approach in practice: creating system backups is a common practice and we can load a particular backup DB of our interest without incurring the rollback delay.
For the SQL transpiler, we implemented the JavaScript instrumentation software based on Jalangi2~\cite{jalangi2}, and used ExpoSE~\cite{Loring:2017} for path constraint resolution. We implemented the DSE analysis software of the server-side \& client-side JavaScript code based on the Chromium browser, Puppeteer API~\cite{puppeteer}, and MITMProxy~\cite{mitmproxy}. We used NodeJS and Python to implement the Z3-to-Python transpiler. \looseness=-1

\para{Test Setup:} We evaluated \ultraverse on Digital Ocean's VM equipped with 8 vCPUs, 16GB RAM, and 640GB SSD. Our evaluation compared three systems: (1) a baseline NodeJS application; (2) a transpiled NodeJS application with application-level transactions converted into compact SQL \texttt{PROCEDURE}s; and (3) a transpiled NodeJS application with query dependency analysis using the retroactive DBMS plugin. We will denote these three systems as \textsf{B}, \textsf{T}, and \textsf{T+D}. \looseness=-1

Test cases were sourced from four BenchBase~\cite{oltp-bench} micro-benchmarks: TPC-C, TATP, Epinions, and SEATS. We converted the Java source code of these benchmarks JavaScript (NodeJS) for testing. The macro-benchmark used was AStore~\cite{astore}, an open-source e-commerce web application using the ExpressJS framework. AStore is comprised of 61 application-level transactions, of which 20 are database-updating transactions. For the 3 systems, we assessed their performance (\autoref{subsec:performance}), overhead (\autoref{subsec:overhead}), and scalability (\autoref{subsec:scalability}), and finally compare \ultraverse with Mahif~\cite{mahif}(\autoref{subsec:comparison}). Due to the space limit, we provide \ultraverse's column-wise \& row-wise analysis details of all benchmarks in \autoref{appendix:benchmarks}.
\looseness=-1




 \subsection{Performance}
\label{subsec:performance}


\para{\textit{What-if} Simulation Speed: } 
We evaluated the baseline, the transpiled, and the \ultraverse versions, using a backup database as the starting point and a transaction history of 1 million queries. Each \textit{what-if} simulation test randomly selected committed past transactions to retroactively remove or add such that they affect the results of about 1\% of their future transactions (i.e., 10,000 out of 1 million transactions). The transaction commit history was then replayed on the backup database with these retroactive modifications.
\looseness=-1

\begin{table}
\renewcommand\arraystretch{1.2}
\centering
\begin{subfigure}[t]{0.49\textwidth}
\centering
{\includegraphics[width=\linewidth]{figures/Total3.pdf}}
\caption{\textit{What-if} simulation runtime for 1 million queries.}
\label{fig:retroactive-operation}
\end{subfigure}

\begin{subtable}[t]{0.49\textwidth}
  %\footnotesize
  \centering  
  \begin{tabular}{|c||c|c|c|c|c|c|}  % left align
    \hline
    % & TPC-C & TATP & Epinions & SEATS & YCSB & RS \\\hline\hline
    % \texttt{S} & 7.0\% & 0.7\% & 3.9\% & 3.9\% & 0.2\% & 6.4\% \\\hline 
    % \texttt{S + H} & 9.5\% & 0.6\% & 4.9\% & 4.2\% & 0.8\% & 6.3\% \\\hline
    & Epinions & TATP & SEATS & TPC-C & AStore \\\hline\hline
    \textbf{at 10\%} & 5s & 52s & 131s & 107s & 8s \\\hline
    \textbf{at 25\%} & 12s & 128s & 65s & 51s & 20s \\\hline
    \textbf{at 50\%} & 23s & 257s & 0.18H & 0.14H & 40s \\\hline
    \textbf{at 100\%} & 46s & 512s & 0.36H & 0.29H & 77s \\\hline
  \end{tabular}
\caption{Hash-jumper's runtime across various hash-hit points.}  
  \label{tab:hash-jumper}
\end{subtable}


\begin{subtable}[t]{0.49\textwidth}
   \footnotesize
  \centering
  \begin{tabular}{|c||c|c|c|c|c|c|}  % left align
    \hline
    % & TPC-C & TATP & Epinions & SEATS & YCSB & RS \\\hline\hline
    % \texttt{S} & 24\% & 99\% & 65\% & 28\% & 0\% & 94\% \\\hline 
    % \texttt{S + H} & 24\% & 99\% & 95\% & 87\% & 0\% & 98\% \\\hline
    & Epinions & TATP & SEATS & TPCC & AStore \\\hline\hline
    \textbf{\textsf{B}} & 1.11ms & 2.62ms & 7.99ms & 32.8ms & 9.1ms \\\hline 
    \textbf{\textsf{T/T+D}} & 1.11ms & 2.06ms & 6.79ms & 8.6ms & 7.1ms \\\hline    
  \end{tabular}
  \caption{Runtime of regular application-level transactions.}  
  \label{tab:regular-transaction-speed}
\end{subtable}

\caption{Performance of \ultraverse.}
\label{tab:performance}
\end{table}

Different replay strategies were adopted for the three systems. The baseline version serially replayed all committed application function calls of the unmodified application-level transactions-- serial execution is necessary to ensure strong serializability of the \textit{what-if} replay. The transpiled version serially replayed the function calls of the transpiled application-level transactions. The \ultraverse version directly replayed the raw SQL \texttt{PROCEDURE}s from the log based on column-wise and row-wise query dependency analysis. \looseness=-1

\autoref{fig:retroactive-operation} compares the runtime of \textit{what-if} simulation for the transaction history window of 1 million queries.
The \textsf{T+D} version was 23.60x faster on average than the baseline version, and the transpiled version was 2.01x faster on average than the \textsf{B} version. The \textsf{T} version gained speed primarily due to the SQL transpilation technique, which merged the calls of individual queries belonging to the same application-level transaction into a single SQL \texttt{PROCEDURE} call, thus reducing the number of round-trip communications between the DBMS client and server. This advantage became more pronounced when each application-level transaction contains a higher number of query executions by using loops (e.g., SEATS, TPC-C, AStore). \looseness=-1
%6891s, 3423s, 292s

The \ultraverse version gained additional speed from column-wise and row-wise query dependency analysis, which reduced the number of queries to replay and increased the level of query execution parallelism during replay. Benchmarks such as Epinions, TATP, and AStore benefited from both replay query reduction and parallel replay. SEATS and TPC-C benefited only from replay parallelism, as all transactions in these two benchmarks depended on the retroactive operation's target transactions in both column-wise and row-wise terms. \looseness=-1

In all three system versions, reading the query log and replaying queries were performed in parallel. However, because the disk batch-reading speed of SSD NVMe was faster than the DBMS's serial execution of queries, the critical path of \textit{what-if} simulation was the DBMS's replay runtime rather than the disk I/O of query logs. \looseness=-1



\para{Hash-jumper: }
The \ultraverse version gains additional speed with its Hash-jumper feature enabled, as shown in \autoref{tab:hash-jumper}. This test, unlike the one referred to in \autoref{fig:retroactive-operation}, used 10 million queries. The Hash-jumper prototype has an upper-bound hash collision rate of approximately {$1.16 x 10^{-77}$}. Each benchmark's test cases were set up to have a hash-hit at various timestamp locations (10\%, 25\%, 50\%, and 100\%) in the transaction history. The sooner a hash-hit was detected by \ultraverse, the sooner the \textit{what-if} replay terminated, finishing the effectless operation. The test case with no hash-hit (i.e., at 100\%) implicitly measures the overhead of enabling Hash-jumper. This overhead was on average 2.4\%, reflected in the slowdown of the replay speed compared to disabling Hash-jumper. However, this overhead can be compensated by increasing the number of CPUs and RAMs, since the hash computation does not require additional disk I/O on the database.



\begin{table}

\begin{subtable}[t]{0.50\textwidth}
  \footnotesize
  \centering
\resizebox{\linewidth}{!}{
  \begin{tabular}{|l||c|c|c|c|c|}  % left align
    \hline
    & Epinions & TATP & SEATS & TPC-C & AStore \\\hline\hline
    \textbf{Analysis Time} & 21.3s & 31.7s & 145.2s & 151.3s & 187.8s \\\hline
  \end{tabular}
  }
  \caption{SQL transpiler's application code analysis time.}
  \label{tab:transpilation} 
\end{subtable}

\begin{subtable}[t]{0.50\textwidth}
   \footnotesize
  \centering
\resizebox{\linewidth}{!}{
  \begin{tabular}{|l||c|c|c|c|c|c|}  % left align
    \hline
    & Epinions & TATP & SEATS & TPC-C & AStore \\\hline\hline
    \textbf{MySQL's Query Log} & 291b & 376b & 524b & 489b & 441b \\\hline
    \textbf{\ultraverse's Log} & 12b & 48b & 35b & 110b & 76b \\\hline
  \end{tabular}
  }
  \caption{Average log size per query (bytes).}
  \label{tab:ultraverse-space-overhead} 
\end{subtable}


\begin{subtable}[t]{0.50\textwidth}
   \footnotesize
  \centering  
  \begin{tabular}{|c||c|c|c|c|c|c|}  % left align
    \hline
    & TPC-C & TATP & Epinions & SEATS & RS \\\hline\hline
    \textbf{\textsf{T+D}} & 7.0\% & 0.7\% & 3.9\% & 3.9\% & 6.4\% \\\hline 
    \textbf{\textsf{T+D+H}} & 9.5\% & 0.7\% & 4.9\% & 4.2\% & 6.4\% \\\hline
  \end{tabular}
  \caption{Query dependency logger's overhead.}  
  \label{tab:logging-overhead}
\end{subtable}

\begin{subtable}[t]{0.50\textwidth}
   \footnotesize
  \centering
\begin{tabular}{|l||c|c|c|c|c|c|}  % left align
    \hline
    & TPC-C & TATP & Epinions & SEATS & AStore \\\hline\hline
    \textbf{Slowdown} & 8.2\% & 7.2\% & 14.1\% & 16.5\% & 13.3\% \\\hline
  \end{tabular}
  \caption{Overhead of simultaneously running \textit{what-if} simulation and regular operations in the same machine.}
  \label{tab:simultaneous-overhead} 
\end{subtable}

\caption{Overhead of \ultraverse.}
\label{tab:overhead}
\end{table}





\para{Regular Transaction Speed: }
\ultraverse's SQL transpiler merges the queries executed separately in an application-level transaction function into a single SQL \texttt{PROCEDURE}, effectively reducing the RTT between the DBMS client and server. This transpilation technique can be used not only for \textit{what-if} analysis, but also for speeding up the processing of regular application-level transactions. \autoref{tab:regular-transaction-speed} compares the average transaction runtime of each benchmark for the baseline and transpiled versions. On average, the baseline version took 10.7ms to process a transaction, whereas the transpiled version took 5.13ms-- 105.1\% faster. 
The speed of Epinions was the same, because its each transaction was a single query. On the other hand, SEATS, TPC-C, and AStore had greater speedup because they had loops of executing multiple queries in a single transaction. 
In this local machine test, the RTT between the DBMS client and server was about 1ms. However, in a remote DBMS setup with a larger RTT (e.g., >20ms), the speedup from the transpiled version would be multiplied by the increase in RTT. Meanwhile, this speedup due to RTT gradually diminishes as each transaction requires more time for local computation (to be discussed in \autoref{subsec:scalability}).
\looseness=-1

\subsection{Overhead}
\label{subsec:overhead}



\para{Transpilation Time: }
The SQL transpilation time consists of application code instrumentation, path exploration with dynamic symbolic execution, and the final conversion into SQL code. As shown in \autoref{tab:transpilation}, the transpilation time for each benchmark varied from 21.3 seconds to 187.8 seconds. This time increased with the number of application-level transactions or the number of execution paths (e.g., loops). Importantly, this transpilation overhead only occurs once per application during offline code analysis. \looseness=-1



\begin{table}[t]
\footnotesize
\centering
\setlength{\tabcolsep}{2.2pt}

\renewcommand\arraystretch{1.2}
\centering
\begin{subtable}{0.49\textwidth}
\centering
\begin{tabular}{|l||ccc|ccc|ccc|}
\toprule
\multirow{2}{*}{
{\textbf{Bench.}}}
  & \multicolumn{3}{c}{\textit{\textbf {History Size: 1M}}} &
\multicolumn{3}{c}{\textit{ \textbf {: 10M}}} & \multicolumn{3}{c|}{\textit{ \textbf {: 100M}}} \\ 
\cmidrule{2-4} \cmidrule{5-7} \cmidrule{8-10}

 &\textsf{B}&\textsf{T}&\textsf{T+D}&\textsf{B}&\textsf{T}&\textsf{T+D}&\textsf{B}&\textsf{T}&\textsf{T+D} \\
\hline
Epinions &1024s&1024s&4s&2.85H&2.85H&45s&28.6H&28.6H&490s\\
TATP &1215s&1030s&45s&3.30H&1.14H&505s&32.9H&11.63H&1.45H\\
SEATS &1422s&371s&130s&3.95H&1.02H&0.36H&39.4H&10.18H&3.60H\\
TPC-C &1426s&405s&116s&3.96H&1.11H&0.29H&39.6H&18.36H&2.91H\\
AStore &1804s&592s&12s&5.02H&1.68H&135s&50.4H&17.01H&0.38H\\
\bottomrule
\end{tabular}
\caption{\textit{What-if} analysis time for various transaction history sizes.}
\label{tab:retroactive-windows}
\end{subtable}
    
\begin{subtable}{0.5\textwidth}
\centering
\begin{tabular}{|l||cc|cc|cc|}
\toprule
\footnotesize
\multirow{2}{*}{
{\textbf{Benchmark}}}
  & \multicolumn{2}{c}{\textit{\textbf {DB Size: 1x}}} &
\multicolumn{2}{c}{\textit{ \textbf {: 5x}}} & \multicolumn{2}{c|}{\textit{ \textbf {: 10x}}} \\ 
\cmidrule{2-3} \cmidrule{4-5} \cmidrule{6-7} &\textsf{T}&\textsf{T+D}&\textsf{T}&\textsf{T+D}&\textsf{T}&\textsf{T+D} \\
\hline
Epinions &1.00x&256x&1.00x&256x&1.00x&256x\\
TATP &1.27x&27.0x&1.27x&26.21x&1.27x&25.8x\\
SEATS &3.84x&11.18x&3.69x&10.85x&3.67x&10.5x\\
TPC-C &3.16x&13.41x&3.03x&12.70x&2.66x&11.45x\\
AStore &3.05x&301x&3.03x&299x&3.02x&291x\\
\bottomrule
\end{tabular}
\caption{Speed against Baseline across various DB sizes.} 
\label{tab:database-sizes} 
\end{subtable}
    
\begin{subtable}{0.5\textwidth}
\centering
\begin{tabular}{|l||cc|cc|cc|cc|}
\toprule
\footnotesize
\multirow{2}{*}{
{\textbf{Benchmark}}}
  & \multicolumn{2}{c}{\textit{\textbf {Dependency: 1\%}}} &
\multicolumn{2}{c}{\textit{ \textbf {: 10\%}}} & \multicolumn{2}{c}{\textit{ \textbf {: 50\%}}} & \multicolumn{2}{c|}{\textit{ \textbf {: 100\%}}} \\ 
\cmidrule{2-3} \cmidrule{4-5} \cmidrule{6-7} \cmidrule{8-9} &\textsf{T}&\textsf{T+D}&\textsf{T}&\textsf{T+D}&\textsf{T}&\textsf{T+D}&\textsf{T}&\textsf{T+D} \\
\hline
Epinions &1.0x&256x&1.0x&35.5x&1.0x&6.7x&1.0x&3.6x\\
TATP &1.3x&27.0x&1.3x&57.7x&1.3x&11.2x&1.3x&4.1x\\
SEATS &-&-&-&-&-&-&3.8x&11.2x\\
TPC-C &-&-&-&-&-&-&3.2x&13.4x\\
AStore &3.1x&301x&3.1x&94.3x&3.1x&18.3&3.1x&9.3x\\
\bottomrule
\end{tabular}
\caption{Speedup against Baseline across various query dependencies.} 
\label{tab:dependency-rates} 
\end{subtable}
\caption{Scalability of \ultraverse.}
\label{tab:comparison}
\end{table}

\para{Query Dependency Log Size: }
\autoref{tab:ultraverse-space-overhead} compares the size of MySQL's binary query log and the additional log generated by \ultraverse. On average, MySQL's binary log is 424 bytes per query, while \ultraverse introduces an additional 56 bytes per query, resulting in a 7.6\% increase in the log storage overhead.
\looseness=-1

\begin{table*}[t]
\setlength{\tabcolsep}{2.5pt}
\footnotesize
\renewcommand\arraystretch{1.2}
\centering
\begin{subtable}{0.49\textwidth}
\centering
\begin{tabular}{|l||cc|cc|cc|cc|}
\toprule
\multirow{2}{*}{
{\textbf{Bench.}}}
  & \multicolumn{2}{c}{\textit{\textbf {250 Queries}}} &
\multicolumn{2}{c}{\textit{ \textbf {500 Queries}}} & \multicolumn{2}{c}{\textit{ \textbf {1K Queries}}} & \multicolumn{2}{c|}{\textit{ \textbf {2K Queries}}} \\ 
\cmidrule{2-3} \cmidrule{4-5} \cmidrule{6-7} \cmidrule{8-9}

 &\textsf{T+D}&\textsf{M}&\textsf{T+D}&\textsf{M}&\textsf{T+D}&\textsf{M}&\textsf{T+D}&\textsf{M} \\
\hline
Epinions &0.7s&82.3s&0.7s&710.2s&0.7s&2.3H&0.7s&>20.8H\\
TATP &0.6s&34.5s&0.6s&254.2s&0.6s&2358s&0.8s&8.3H\\
SEATS &1.4s&$\times$&1.7s&$\times$&1.9s&$\times$&2.9s&$\times$\\
TPC-C &1.3s&23.8s&1.5s&167.2s&1.6s&1387s&2.4s&4.3H\\
AStore &0.7s&37.7s&0.7s&291.2s&0.7s&2824s&0.7s&10.1H\\
\bottomrule
\end{tabular}
\caption{\textit{What-if} analysis time comparison (``$\times$" means N/A)}\label{tab:comparison-speed}
\end{subtable}
    \hfil
\begin{subtable}{0.49\textwidth}
\centering
\begin{tabular}{|l||cc|cc|cc|cc|}
\toprule
\multirow{2}{*}{
{\textbf{Bench.}}}
  & \multicolumn{2}{c}{\textit{\textbf {250 Queries}}} &
\multicolumn{2}{c}{\textit{ \textbf {500 Queries}}} & \multicolumn{2}{c}{\textit{ \textbf {1K Queries}}}  & \multicolumn{2}{c|}{\textit{ \textbf {2K Queries}}}  \\ 
\cmidrule{2-3} \cmidrule{4-5} \cmidrule{6-7} \cmidrule{8-9}

 &\textsf{T+D}&\textsf{M}&\textsf{T+D}&\textsf{M}&\textsf{T+D}&\textsf{M}&\textsf{T+D}&\textsf{M} \\
\hline
Epinions &43MB&3.5GB&43MB&10.9GB&48MB&40.8GB&54MB&>126GB\\
TATP &43MB&2.8GB&43MB&8.1GB&48MB&29.2GB&54MB&111GB\\
SEATS &43MB&$\times$&56MB&$\times$&71MB&$\times$&92MB&$\times$\\
TPC-C &43MB&1.9GB&54MB&6.0GB&64MB&23.4GB&88MB&87.8GB\\
AStore &43MB&2.8GB&46MB&7.9GB&49MB&25.6GB&61MB&90.2GB\\
\bottomrule
\end{tabular}
\caption{RAM overhead comparison} 
\label{tab:comparison-overhead}
\end{subtable}

\caption{Comparison between \ultraverse (\textsf{T+D}) and Mahif~\cite{mahif} (\textsf{M})  across various transaction history sizes (250$\sim$-2K queries).}
\label{tab:comparison2}
\end{table*}



\para{Logging Read/Write Sets and Hashes: }
During regular operations, \ultraverse's DBMS plugin runs an asynchronous background process that infers column-wise and row-wise $R$/$W$ sets of committed queries and table hashes. This incurs additional computational overhead. The overhead this background logging activity imposes on the regular query processing operation of the DBMS is measured in \autoref{tab:logging-overhead}, where \textsf{T+D} refers to the \ultraverse version and \textsf{T+D+H} refers to \ultraverse with Hash-jumper enabled. Across all benchmarks, the overhead from the logging activity ranged from 0.6\% to 9.5\%. However, this overhead can be offset in a practical setting by copying the DBMS's MySQL binary log to another machine and having \ultraverse generate its $R$/$W$ set logs on that machine. This is feasible because \ultraverse's logging daemon operates asynchronously and independently from the DBMS's regular operations.
\looseness=-1


\para{Concurrent \textit{What-if} Simulation with Regular Operations: }
The impact on the DBMS's regular operations while the \textit{what-if} simulation is concurrently running in the background is shown in \autoref{tab:simultaneous-overhead}. The average slowdown overhead ranged from 3.3\% to 16.5\%. This overhead can also be reimbursed if the \textit{what-if} simulation is run on a different machine, using a copied backup database and transaction history.
\looseness=-1


\subsection{Scalability}
\label{subsec:scalability}





\noindent\textbf{Transaction History Size: }
The runtime of the \textit{what-if} simulation was measured across different transaction history sizes: 1M, 10M, and 100M queries. \autoref{tab:retroactive-windows} compares the runtimes of the three versions (i.e., baseline, transpiled, and \ultraverse). The runtimes of all three systems increased proportionally with the size of the transaction history, as their number of transactions to replay also increased linearly.
\looseness=-1

\para{Database Size: }
The runtime of the \textit{what-if} simulation was also measured across different database sizes: 1x, 5x, and 10x,  ranging from 10MB to 10GB in overall. The speedup of the transpiled and \ultraverse versions compared to the baseline version is shown in \autoref{tab:database-sizes}. The speedup remained generally consistent as the database size increased. However, benchmarks with computationally intensive transactions, such as SEATS and TPC-C, experienced more significant slowdowns. This occurred because the benefits of RTT reduction from transpilation were degraded by the increased computational time for transactions due to the increased database size (e.g., larger tables took more time for JOIN operations). \looseness=-1

\para{Query Dependency Rate: }
The runtime of the \textit{what-if} simulation was measured across different query dependency rates: 1\%, 10\%, 50\%, and 100\%. The speed of the baseline and transpiled versions remained the same regardless of changes in the query dependency rate since they had to replay all queries in the transaction history, anyway. For the \ultraverse version, as the query dependency rate increased and it had to replay more queries than before, the speedup rate decreased. However, even when the dependency rate was 100\% (requiring the replay of all queries), the \ultraverse version was still faster than the baseline and transpiled versions. This is because query dependency analysis enabled the parallel replay of multiple queries with non-conflicting $R$/$W$ sets, resulting in a speedup ranging from 2.7x to 4.2x. For the SEATS and TPC-C benchmarks, we report only for a 100\% query dependency rate, because in those benchmarks almost all transactions depended on each other over the long run due their complex data record correlations. However, it's important to note that their multiple consecutive queries could still be replayed in parallel if their column-wise or row-wise $R$/$W$ sets had no \textit{read-write}, \textit{write-write}, and \textit{write-read} conflicts. \looseness=-1




%\subsection{Other Use Cases}
%\label{subsec:case-study}

%The \ultraverse system also offers a unique solution for ensuring GDPR compliance in data analytics. The typical modern data analytics architectures, such as Azure~\cite{olap1} or IBM Analytics~\cite{olap2}, follow a four-stage process: \textit{(i)} sourcing data; \textit{(ii)} storing data in an SQL database; \textit{(iii)} retrieving and processing data records to create materialized views; \textit{(iv)} using these materialized views to execute various data analytics operations.
%GDPR regulations stipulate that when a user requests data deletion, all data records derived from the user's data during analytics must also be updated. This means that the third stage (data processing) must be replayed to apply changes to the materialized views. However, this stage often involves complex and computationally intensive machine learning or advanced statistical algorithms, which often do not have efficient incremental deletion algorithms. This is where \ultraverse comes into play, providing an efficient method to update materialized views in compliance with GDPR data deletion requirements.
%The system can be readily integrated into many data analytics frameworks such as Hive~\cite{hive}  or Spark SQL~\cite{sparkql}, which already support SQL for implementing complex data processing logic.

%The effectiveness of \ultraverse was demonstrated in a common data analytics scenario that runs the K-clustering algorithm on 1 million online articles created by 10,000 users. These articles are classified into 10 categories based on word relevance using the LDA algorithm~\cite{lda}. The stage for data processing and view materialization utilized Hive~\cite{hive} and Hivemall~\cite{hivemall}, a machine learning programming framework that relies on JDBC.
%The application was ported into \ultraverse, and the replay time was compared with and without dependency analysis. The average overhead of \ultraverse during regular service operations was 1.8\%, and the speedup in retroactive operations was 41.7x. This significant speedup resulted from the elimination of independent queries in the article classification stage, where each user ID acted as the RI key.




\subsection{Comparison with Mahif}
\label{subsec:comparison}



To evaluate \ultraverse's effectiveness, we compared it to Mahif~\cite{mahif}, a cutting-edge \textit{what-if} DBMS. In particular, we used the open-source Mahif prototype~\cite{mahif-prototype}. Because Mahif demands a considerable amount of memory, we conducted the comparison on a bigger virtual machine with 12 CPU cores and 128GB RAM. As Mahif can only support a limited number of historical queries, we compared it to \ultraverse using transaction histories of 250, 500, 1000, and 2000 queries. Due to Mahif's inability to support string attributes, we were unable to provide data for the SEATS benchmark for Mahif, since all the \texttt{UPDATE/DELETE/INSERT} queries in SEATS involved string attributes (marked as $\times$ in the tables). 
\textcolor{orange}{We tested Mahif only up to 2,000 queries is because Mahif is not scalable over the transaction history size and cannot practically replay 1M, 10M, or 100M queries (which is expected to take $>$ 30,000 hours and consume $>$ 48,000TB RAM).}
\looseness=-1

\para{\textit{What-if} Answering Speed: } \autoref{tab:comparison-speed} compares the \textit{what-if} analysis speed of \ultraverse and Mahif. In overall, \ultraverse (0.6s$\sim$2.9s) was 6450x faster than Mahif (23.8s$\sim$20.8H). The reason is because Mahif's runtime overhead increased exponentially as the number of historical queries increased, due to its growth of symbolic expression costs. On the other hand, \ultraverse only needed to parse and analyze the dependency of each query and replay only the dependent queries.  \looseness=-1

\para{Overhead: } \autoref{tab:comparison-overhead} compares the memory usage of \ultraverse and Mahif. In overall, \ultraverse (43$\sim$92MB) was 1370x more memory-efficient than Mahif (requiring 2.8G$\sim$126GB). The memory required by \ultraverse is primarily used for temporarily storing each query statement, replaying each dependent query, and maintaining the dependent $R/W$ sets, while Mahif required an exponentially growing amount of memory with the number of queries. \looseness=-1

\para{Correctness: } Unlike \ultraverse, Mahif failed to maintain the accuracy of application-level semantics during its \textit{what-if} simulation for TPC-C, SEATS, and TPCC transactions, because Mahif's analysis only handles SQL queries and does not capture the application-level logic. Moreover, Mahif's \textit{what-if} analysis does not support the use of SQL \texttt{TRANSACTION}/\texttt{PROCEDURE}. Mahif also lacked support for certain SQL features and query types, such as using string, boolean, or date/time type as column attributes, native SQL APIs (e.g., \texttt{CURRENT\_TIMESTAMP()} or \texttt{RANDOM()}), or DML (\texttt{CREATE, DROP, ALTER}) queries. Due to these reasons, Mahif didn't preserve the correctness of \textit{what-if} analysis in application-level or SQL-level transactions. \looseness=-1



==> introduction-dbms.tex <==
\section{Introduction}
\label{sec:introduction}

\textit{What-if} analysis is a technique to hypothetically alter data records or actions in transaction history and model predicted outcomes in a new simulation context. This technique proves beneficial in various scenarios, including data analytics, software performance tuning, risk management, program testing/debugging, and the cleanup of corrupt past transactions or data~\cite{what-if-survery1, what-if-survery2}.




%Today's majority of software use database systems (DBMS) as persistent storage. 
In recent decades, numerous \textit{what-if} DBMS techniques \cite{mahif, caravan, tiresias, qfix, whatif1, whatif2, whatif3} have emerged to efficiently manage \textit{what-if} database queries. However, these methods often fall short in real-world software applications since they only factor in database queries, neglecting the impact of data flows in application code affecting the database's state. Notably, most contemporary software is implemented using various application languages, not exclusively SQL.

\begin{figure}
\begin{scriptsize}
\begin{Verbatim}[frame=single, baselinestretch=0.7, commandchars=\\\{\}]
\textcolor{blue}{{1: }}\textbf{function} NewFollows \textbf{(}src_user, dst_user\textbf{):} 
\textcolor{blue}{{2: }}   \textbf{var} result_rows \textbf{=} \textbf{SQL_exec(}\textit{\textcolor{brown}{"SELECT COUNT(*)  FROM Blocks}}
\textcolor{blue}{{3: }}    \textit{\textcolor{brown}{ WHERE src_uid = "}} \textbf{+} src_user \textbf{+} \textit{\textcolor{brown}{ AND dst_uid = "}} \textbf{+} dst_user\textbf{);}
\textcolor{blue}{{4: }}   \textbf{if (}result_rows[0]['COUNT(*)'] \textbf{>} 0\textbf{)}
\textcolor{blue}{{5: }}      \textbf{return} "Error: User " + dst_user + " is blocked"\textbf{;}
\textcolor{blue}{{6: }}   \textbf{else} 
\textcolor{blue}{{7: }}       \textbf{SQL_exec(}\textcolor{brown}{"INSERT INTO Follows (src_uid, dst_uid) VALUES ("}
\textcolor{blue}{{8: }}        + src_user + \textcolor{brown}{", "} + dst_user + \textcolor{brown}{")"}\textbf{);}
\end{Verbatim}
\end{scriptsize}
\caption{A social networking server's user request handler.}
\label{fig:new-follows-code}
\end{figure}

\autoref{fig:new-follows-code} illustrates this issue using JavaScript application code. It displays a web server's handler function (a simplified version), where the \texttt{NewFollows} function responds to a user request to follow another user. This function represents an \textit{application-level} transaction consisting of two SQL queries. The first \texttt{SELECT} query verifies if the requesting user blocked the target user in the past. If not, the second \texttt{INSERT} query establishes a social networking connection to the target user. Assume that we intend to conduct an application-level \textit{what-if} analysis that involves removing a past \texttt{BlockUser} transaction and simulating the resultant final application state.
Current DBMS-oriented \textit{what-if} analysis techniques fail to perform such application-level \textit{what-if} analyses as they do not analyze the software logic incorporated at the application code layer. Specifically, during the \textit{what-if} analysis, the \texttt{if} statement of some \texttt{NewFollows} call might traverse the \texttt{false} branch instead of the \texttt{true} branch due to the removal of a user-blocking transaction. However, existing DBMS-based query replay techniques disregard the application code's control flow logic or data flows that can impact the database's state. As a result, their \textit{what-if} analysis, excluding the application logic, leads to inaccurate results from the application's viewpoint.

While other research work focused on application attack recovery and forensics~\cite{warp, rail, chromepic, regexnet} manages to avoid this problem by replaying both the application code and their associated DBMS queries, these approaches often lack scalability. For instance, given that each headless (graphic-less) Chromium browser instance requires around 100MB of RAM, the \textit{what-if} analysis overhead for a large user base (say, 1 million) becomes practically infeasible. 
Such scalability is also a prominent issue in \textit{what-if} DBMSes. Mahif~\cite{mahif}, the state-of-the-art DBMS for historical \textit{what-if} queries of the four basic types (\texttt{INSERT}, \texttt{UPDATE}, \texttt{DELETE}, and \texttt{SELECT}), exhibits this problem. The system's resource consumption increases exponentially with the linear growth of the transaction history size, rendering it incapable of processing a transaction history that contains more than 2,000 SQL queries (\autoref{subsec:comparison}). 


To address the requirements of accuracy in application-wide \textit{what-if} analysis and scalability, we introduce \ultraverse, an efficient framework for application-level \textit{what-if} analysis. Conventionally, \textit{what-if} analysis is akin to a "retroactive operation" that modifies a \textit{past} operation in a series of committed ones, such as cancelling a previously committed insertion of '5' into a queue at time \textit{t=3}. Previous research has explored retroactive operations on fundamental data structures like queues~\cite{retroactive-queue}, doubly linked queues~\cite{retroactive-dqueue}, priority queues~\cite{retroactive-pqueue}, and union-find structures~\cite{retroactive-ufind}.
\ultraverse stands out as the first DBMS to efficiently support retroactive operations on both SQL queries and application-level transactions while preserving the correctness of both SQL-level and application-level semantics. It consists of two components: \textbf{(1) An SQL transpiler} transforms application code into its equivalent concise SQL procedures; and \textbf{(2) A retroactive operation DBMS plugin} efficiently executes \textit{what-if} analysis on the transpiled SQL procedures.

%\begin{itemize}
%    \item 
    \para{SQL Transpiler (\autoref{sec:transpiler})} translates each transaction of a target application (developed in application languages) into a compact SQL \texttt{PROCEDURE}, which only contains data flows that update the persistent database storage. \ultraverse replays these transpiled \texttt{PROCEDURE}s rather than the original application code, ensuring a faster replay speed. This is due to the transpiler's pruning of application logic that doesn't affect persistent storage. Additionally, the transpiler consolidates multiple SQL queries within the same application-level transaction into a single SQL \texttt{PROCEDURE}, thereby reducing round-trip communications between the DBMS client and server. In the \autoref{fig:new-follows-code} example, the transpiled code would include the \texttt{SELECT} and \texttt{INSERT} queries within one \texttt{PROCEDURE}, reducing the round-trip time (RTT) from two to one. This reduction becomes even more significant when an application-level transaction uses loops to execute a larger number of individual SQL queries, as all these queries will execute within a single RTT as part of the single \texttt{PROCEDURE} call. The \ultraverse SQL transpiler is compatible with legacy application code and doesn't require manual modifications by developers. However, it faces the significant challenge of transpiling modern application languages (like JavaScript, PHP) with dynamic features that are difficult to analyze statically, such as dynamic variable type resolution, modifiable function pointers as object properties, asynchronous event calls, etc. Converting such dynamic behaviors into semantically equivalent SQL code is non-trivial. To address this, \ultraverse's transpiler utilizes dynamic symbolic execution (\autoref{subsec:dse}).

    %\item 
    \para{Retroactive Operation DBMS Plugin (\autoref{sec:design})} performs query dependency analysis on the SQL \texttt{PROCEDURE} code produced by the SQL transpiler. This analysis occurs in two orthogonal aspects: column-wise (\autoref{subsec:columnwise-dependency-analysis}) and row-wise (\autoref{subsec:rowwise-analysis}) analysis, which respectively consider all the table columns and rows each query could potentially read or write. Based on the static read-write dependency analysis of the queries, \ultraverse excludes queries for replay whose execution results are deterministically unaffected by the modified \textit{what-if} target query (or queries). This step reduces the number of queries to be replayed. Additionally, \ultraverse safely runs multiple queries concurrently if their read/write sets have no conflicts, further accelerating the replay. To further improve the speed, \ultraverse introduces the Hash-jumper technique(\autoref{subsec:hashjump}) which computes each table's state as a hash (to track its change in state) upon each query commit and uses these hashes to decide whether to skip unnecessary replay during \textit{what-if} analysis (i.e., when it detects a table's hash match between the regular operation and the retroactive operation). \ultraverse is compatible with unmodified DBMSes that support SQL, enhancing its practical deployability. \ultraverse supports rich SQL semantics\footnote{\ultraverse supports DDL (schema updates), transactions, stored procedures, triggers, control flow branches, temporary variables, and native APIs.}(\autoref{subsec:columnwise-dependency-analysis}), which are mostly unsupported by prior \textit{what-if} DBMSes.
%\end{itemize}

We have implemented \ultraverse and evaluated its \textit{what-if} analysis performance against a baseline application built with NodeJS + MySQL. Across various BenchBase benchmarks \cite{oltp-bench} (TPC-C, TATP, Epinions, and SEATS), \ultraverse exhibited a speedup ranging from 7.7x to 512x (\autoref{subsec:performance}), and was found to be 6450x faster than Mahif \cite{mahif} (\autoref{subsec:comparison}). We also tested \ultraverse on an open-source e-commerce web application (AStore \cite{astore})\ignore{ and machine-learning data analytics (Apache Hivemall \cite{hivemall})}, with \ultraverse achieving a \textit{what-if} analysis speedup between 18.7x and 601x. The space overhead for \textit{what-if} analysis using \ultraverse is marginal, e.g., 12 to 110 bytes for the log size per query, in contrast to hundreds of bytes for MySQL's query log. 

\para{Contributions}. Our work makes the following contributions:
\begin{itemize}
\item We design an efficient general-purpose retroactive DBMS.
\item We develop an efficient application-level \textit{what-if} analysis framework preserving both application-level and SQL-level semantics.
\item We implement and demonstrate the efficiency of the \ultraverse prototype through an empirical evaluation.
\end{itemize}




==> savespace-ultimate.tex <==
\usepackage[all=normal, floats, bibnotes, wordspacing, charwidths, indent, lists]{savetrees}
\makeatletter%
\captionsetup{belowskip=0pt}



\usepackage{hyperref}
\renewcommand{\sectionautorefname}{\S\@gobble}
\renewcommand{\subsectionautorefname}{\S\@gobble}
\renewcommand{\appendixautorefname}{\S\@gobble}
%\renewcommand{\figureautorefname}{foo}
%\renewcommand{\tableautorefname}{bar}

\skip\footins 0.5\baselineskip %8.1pt plus 4pt minus 2pt
\floatsep 0.5\baselineskip
\textfloatsep 0.5\baselineskip
\intextsep 0.5\baselineskip 
\dbltextfloatsep 0.5\baselineskip  
\dblfloatsep 0.5\baselineskip 

\raggedbottom

\belowcaptionskip 0pt

\usepackage{longtable}
\setlength\LTpre{0.5\baselineskip}
\setlength\LTpost{0.5\baselineskip}

\usepackage{titlesec}
\titlespacing\section{0pt}{0.5\baselineskip}{0pt}
\titlespacing\subsection{0pt}{0.5\baselineskip}{0pt}
\titlespacing\subsubsection{0pt}{0pt}{0pt}

\everypar{\looseness=-1 }

%%% Include this only if the ACM style is used %%%
%\captionsetup[table]{position=bottom}
\setlength{\abovecaptionskip}{0pt} % 
%\setlength{\belowcaptionskip}{-\baselineskip} 
%\addtolength{\belowcaptionskip}{1ex}

==> savespace.tex <==
\usepackage[all=normal, floats, bibnotes, wordspacing, charwidths, indent, lists]{savetrees}
\makeatletter%
\captionsetup{belowskip=0pt}



\usepackage{hyperref}
\renewcommand{\sectionautorefname}{\S\@gobble}
\renewcommand{\subsectionautorefname}{\S\@gobble}
\renewcommand{\appendixautorefname}{\S\@gobble}
%\renewcommand{\figureautorefname}{foo}
%\renewcommand{\tableautorefname}{bar}

\skip\footins 0.5\baselineskip %8.1pt plus 4pt minus 2pt
\floatsep 0.5\baselineskip
\textfloatsep 0.5\baselineskip
\intextsep 0.5\baselineskip 
\dbltextfloatsep 0.5\baselineskip  
\dblfloatsep 0.5\baselineskip 

%\raggedbottom

\belowcaptionskip 0pt

%\usepackage{longtable}
%\setlength\LTpre{0.5\baselineskip}
%\setlength\LTpost{0.5\baselineskip}

%\usepackage{titlesec}
%\usepackage[T1]{fontenc}
%\titleformat{0pt}[display]{\MakeUppercase}
%\titlespacing\section{0pt}{0.75\baselineskip}{0.25\baselineskip}
%\titlespacing\subsection{0pt}{0.75\baselineskip}{0.25\baselineskip}
%\titlespacing\subsubsection{0pt}{0pt}{0pt}

\everypar{\looseness=-1 }

%%% Include this only if the ACM style is used %%%
%\captionsetup[table]{position=bottom}
\setlength{\abovecaptionskip}{0pt} % 
%\setlength{\belowcaptionskip}{-\baselineskip} 
%\addtolength{\belowcaptionskip}{1ex}

\widowpenalty=0
\clubpenalty=0

==> scratch.tex <==

\begin{table*}[t!]
 \begin{subfigure}{\linewidth}
\centering
\begin{tabular}{|c|c||c|c|c|c|c|c|c|}
\hline
&&\textbf{Execution}&\textbf{Retroactive}&Dependency&Rollback&Redo&DB-Transform&Redone\\
&&\textbf{Time}&\textbf{DB-Transform}&Analysis&&&Overhead&Queries\\
\hline
\hline
\textbf{TPC-C}&MariaDB&&&-&&&-&\\
\cline{2-9}
\cite{tpcc}&Stitch&&&&&&&\\
\hline
\hline
\textbf{YCSB}&MariaDB&&&-&&&-&\\
\cline{2-9}
\cite{ycsb}&Stitch&&&&&&&\\
\hline
\hline
\textbf{TATP}&MariaDB&&&-&&&-&\\
\cline{2-9}
\cite{tatp}&Stitch&&&&&&&\\
\hline
\hline
\textbf{Sysbench}&MariaDB&&&-&&&-&\\
\cline{2-9}
\cite{sysbench}&Stitch&&&&&&&\\
\hline
\hline
\textbf{Twitter}&MariaDB&&&-&&&-&\\
\cline{2-9}
\cite{oltp-bench}&Stitch&&&&&&&\\
\hline
\end{tabular}
  \caption{Micro Benchmarks on TPC-C, YCSB, TATP, Sysbench, and Twitter.\\$ $}
 \label{tab:micro}
 \end{subfigure}
  \begin{subfigure}{\linewidth}
\centering
\begin{tabular}{|c|c||c|c|c|c|c|c|c|}
\hline
&&\textbf{Normal}&\textbf{Retroactive}&Dependency&Rollback&Redo&DB-Transform&Redone\\
&&\textbf{Throughput}&\textbf{DB-Transform}&Analysis&&& Overhead&Queries\\
\hline
\hline
\textbf{Zabacus}&MariaDB&&&-&&&-&\\
\cline{2-9}
\textbf{Case 1}&Stitch&&&&&&&\\
\cline{2-9}
&Stitch+H&&&&&&&\\
\hline
\hline
\textbf{Zabacus}&MariaDB&&&-&&&-&\\
\cline{2-9}
\textbf{Case 2}&Stitch&&&&&&&\\
\cline{2-9}
&Stitch+H&&&&&&&\\
\hline
\hline
\textbf{Zabacus}&MariaDB&&&-&&&-&\\
\cline{2-9}
\textbf{Case 3}&Stitch&&&&&&&\\
\cline{2-9}
&Stitch+H&&&&&&&\\
\hline
\end{tabular}
  \caption{Macro Benchmarks on three realistic scenarios of the Zabacus web service.}
 \label{tab:micro}
 \end{subfigure}
  \caption{Comparing the delay overhead of MariaDB and Stitch for DB transformation and normal SQL execution.}
  \label{tab:performance}
\end{table*}

%\begin{table*}[t!]
%\centering
%\begin{tabular}{|c|c||c|c|c|c|c|c|}
%\hline
%&&\textbf{Execution}&\textbf{DB-Transform}&Dependency&Rollback&Redo&\textbf{Redone}\\
%&&\textbf{Time}&\textbf{Time}&Analysis&&&\textbf{Queries}\\
%\hline
%\hline
%\textbf{Zabacus}&MariaDB&&&-&&&\\
%\cline{2-8}
%\textbf{Case 1}&Stitch&&&&&&\\
%\cline{2-8}
%&Stitch+H&&&&&&\\
%\hline
%\hline
%\textbf{Zabacus}&MariaDB&&&-&&&\\
%\cline{2-8}
%\textbf{Case 2}&Stitch&&&&&&\\
%\cline{2-8}
%&Stitch+H&&&&&&\\
%\hline
%\hline
%\textbf{Zabacus}&MariaDB&&&-&&&\\
%\cline{2-8}
%\textbf{Case 3}&Stitch&&&&&&\\
%\cline{2-8}
%&Stitch+H&&&&&&\\
%\hline
%\end{tabular}
%  \caption{Macro-benchmarks results of MariaDB, Stitch, and Stitch with Hash Jump.}
%   \label{tab:performance-macro}
%\end{table*}

==> scratch2.tex <==
\begin{table*}[t!]
\centering
\begin{tabular}{|c|c||c|c|c|c|c|c|}
\hline
&&\textbf{Execution}&\textbf{DB-Transform}&Dependency&Rollback&Redo&\textbf{Redone}\\
&&\textbf{Time}&\textbf{Time}&Analysis&&&\textbf{Queries}\\
\hline
\hline
\textbf{TATP}&MariaDB&&&-&&&\\
\cline{2-8}
&Stitch&&&&&&\\
\cline{2-8}
&Stitch+H&&&&&&\\
\hline
\hline
\textbf{espions}&MariaDB&&&-&&&\\
\cline{2-8}
&Stitch&&&&&&\\
\cline{2-8}
&Stitch+H&&&&&&\\
\hline
\hline
\textbf{seat}&MariaDB&&&-&&&\\
\cline{2-8}
&Stitch&&&&&&\\
\cline{2-8}
&Stitch+H&&&&&&\\
\hline
\hline
\textbf{resource-}&MariaDB&&&-&&&\\
\cline{2-8}
\textbf{pressure}&Stitch&&&&&&\\
\cline{2-8}
&Stitch+H&&&&&&\\
\hline
\hline
%\textbf{smallbank}&MariaDB&&&-&&&\\
%\cline{2-8}
%\cite{oltp-bench}&Stitch&&&&&&\\
%\hline
%\hline
%\hline
\textbf{YCSB}&MariaDB&&&-&&&\\
\cline{2-8}
&Stitch&&&&&&\\
\cline{2-8}
&Stitch+H&&&&&&\\
\hline
\hline
\textbf{TPCC}&MariaDB&&&-&&&\\
\cline{2-8}
&Stitch&&&&&&\\
\cline{2-8}
&Stitch+H&&&&&&\\
\hline
\end{tabular}
  \caption{Macro-benchmark results of MariaDB, Stitch, and Stitch with Hash Jumper for retroactive DB transformation.}
   \label{tab:performance-micro}
\end{table*}


<Notes>
- "Transpiled Code Size": SQL transpiler can expand the code size, due to spawning new explicitly written code for each execution path. The final transpiled code is a big tree with if-statements at branching nodes. Its size is larger than the original code. 
- 
- "Non-deterministic APIs": for black box API simulation, we evaluate the easier option: the analyst's handcoding the return value of each API call. 
- "Resolving Types": track types dynamically and create a dynamic type coercion logic. Ultraverse's transpiler can map the following 8 JavaScript variable types to MySQL variable types as follows:
  Null --> NULL
  Undefined --> NULL
  Boolean --> BOOL
  Number --> DOUBLE
  BigInt --> BIGINT
  String --> VARCHAR
  object --> its fields are tracked as symbols of one of the types above. 
  Symbol --> Not Supported
- "Asynchronous Calls": Currently unsupported, but we can do DSE on asynchronous calls, and incorporate its analysis result (i.e., partial path execution tree) into the main path execution tree. 


==> vldbblock.tex <==
%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\pagestyle{\vldbpagestyle}
\begingroup\small\noindent\raggedright\textbf{PVLDB Reference Format:}\\
\vldbauthors. \vldbtitle. PVLDB, \vldbvolume(\vldbissue): \vldbpages, \vldbyear.\\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi}
\endgroup
\begingroup
\renewcommand\thefootnote{}\footnote{\noindent
This work is licensed under the Creative Commons BY-NC-ND 4.0 International License. Visit \url{https://creativecommons.org/licenses/by-nc-nd/4.0/} to view a copy of this license. For any use beyond those covered by this license, obtain permission by emailing \href{mailto:info@vldb.org}{info@vldb.org}. Copyright is held by the owner/author(s). Publication rights licensed to the VLDB Endowment. \\
\raggedright Proceedings of the VLDB Endowment, Vol. \vldbvolume, No. \vldbissue\ %
ISSN 2150-8097. \\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi} \\
}\addtocounter{footnote}{-1}\endgroup
%%% VLDB block end %%%

%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\ifdefempty{\vldbavailabilityurl}{}{
\vspace{.3cm}
\begingroup\small\noindent\raggedright\textbf{PVLDB Artifact Availability:}\\
The source code, data, and/or other artifacts have been made available at \url{https://github.com/dsegszu/privbench}.
\endgroup
}
%%% VLDB block end %%%
